Maintaining Plasticity in Continual Learning via Regenerative Regularization

In continual learning, plasticity refers to the ability of an agent to quickly adapt to new information. Neural networks are known to lose plasticity when processing non-stationary data streams. In this paper, we propose L2 Init, a simple approach for maintaining plasticity by incorporating in the loss function L2 regularization toward initial parameters. This is very similar to standard L2 regularization (L2), the only difference being that L2 regularizes toward the origin. L2 Init is simple to implement and requires selecting only a single hyper-parameter. The motivation for this method is the same as that of methods that reset neurons or parameter values. Intuitively, when recent losses are insensitive to particular parameters, these parameters should drift toward their initial values. This prepares parameters to adapt quickly to new tasks. On problems representative of different types of nonstationarity in continual supervised learning, we demonstrate that L2 Init most consistently mitigates plasticity loss compared to previously proposed approaches.

==> sections/impact_statement.tex <==
\section*{Impact Statement}
Maintaining plasticity in continual learning has implications for the development of adaptable and lifelong learning AI systems. Such systems may be useful in a variety of applications, such as in personalized education where AI systems can adapt to an individual's evolving knowledge and skills, or in healthcare, where continual learning models could improve diagnosis and patient monitoring. However, some negative implications include overfitting to new data, unintended learning or behavior, and difficulty in ensuring stabililty and reliability. For instance, systems with high plasticity might learn from spurious or unintended signals in their environment, leading to the development of behaviors or patterns that were not intended by the designers. Further, high plasticity can lead to instability, where the system changes too rapidly, making it difficult to ensure consistent and reliable performance over time. Such potential consequences must be addressed in future research before adopting continual learning systems broadly.
